How Does Message Passing Improve Collaborative Filtering?

Collaborative filtering (CF) has exhibited prominent results for recommender systems and been broadly utilized for real-world applications. A branch of research enhances CF methods by message passing used in graph neural networks, due to its strong capabilities of extracting knowledge from graph-structured data, like user-item bipartite graphs that naturally exist in CF. They assume that message passing helps CF methods in a manner akin to its benefits for graph-based learning tasks in general. However, even though message passing empirically improves CF, whether or not this assumption is correct still needs verification. To address this gap, we formally investigate why message passing helps CF from multiple perspectives and show that many assumptions made by previous works are not entirely accurate. With our curated ablation studies and theoretical analyses, we discover that (1) message passing improves the CF performance primarily by additional representations passed from neighbors during the forward pass instead of additional gradient updates to neighbor representations during the model back-propagation and (ii) message passing usually helps low-degree nodes more than high-degree nodes. Utilizing these novel findings, we present Test-time Aggregation for CF, namely TAG-CF, a test-time augmentation framework that only conducts message passing once at inference time. The key novelty of TAG-CF is that it effectively utilizes graph knowledge while circumventing most of notorious computational overheads of message passing. Besides, TAG-CF is extremely versatile can be used as a plug-and-play module to enhance representations trained by different CF supervision signals. Evaluated on six datasets, TAG-CF consistently improves the recommendation performance of CF methods without graph by up to 39.2% on cold users and 31.7% on all users, with little to no extra computational overheads.

==> table_dataset.tex <==
\begin{table}[h]
    \centering
    \caption{Dataset Statistics. Due to privacy constrains, we only report approximated values for \texttt{Internal} dataset.}
    \begin{tabular}{l|cccc}
    \toprule 
    Dataset & \# Users & \# Items & \# Interactions & Sparsity \\
    \cmidrule(r){1-5} 
     \texttt{Amazon-book}            & 52,643  & 40,981  & 2,984,108 & 99.94\% \\
     \texttt{Anime}        & 73,515  & 12,295  & 7,813,727 & 99.13\%  \\
     \texttt{Gowalla}          & 29,858 & 40,981  & 1,027,370 & 99.91\%  \\
     \texttt{Yelp-2018}         & 31,668 & 38,048 & 1,561,406 & 99.87\%  \\
     \texttt{Internal}    &  $\sim$0.5M & $\sim$0.2M & $\sim$7M & 99.99\% \\
    \bottomrule
    \end{tabular}
    \label{tab:dataset}
\end{table}

==> table_rebuttal_2.tex <==
\begin{table*}
\begin{center}
\caption{Recommendation performance (i.e., NDCG@10/20 and  Recall@10/20) of efficient matrix factorization methods and performance improvement (\%) of \method over them. Setting explored in this table is the same as what \cref{tab:mftagcf} has. For methods that directly outputs ranking predictions per user, we use an user-derived propagation matrix to conduct test-time augmentation. 
} 
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{l|cc>{\columncolor[gray]{0.9}}c|cc>{\columncolor[gray]{0.9}}c|cc>{\columncolor[gray]{0.9}}c|cc>{\columncolor[gray]{0.9}}c}
\toprule
% \toprule
Metrics & GF-CF & +TAG-CF & Impr. ($\uparrow$) & SVD-GCN-S & +TAG-CF & Impr. ($\uparrow$\%) & SVD-AE & +TAG-CF & Impr. ($\uparrow$\%) & Turbo-CF & +TAG-CF & Impr. ($\uparrow$\%) \\
\bottomrule
\multicolumn{13}{c}{\textsc{Amazon-book}} \\
\cmidrule(r){1-13}  
Recall@10 &7.31 &7.93 &8.5\% &6.72 &6.88 &2.5\% &6.74 &7.23 &7.3\% &7.37 &7.70 &4.4\% \\
NDCG@10 &4.37 &4.75 &8.6\% &3.99 &4.10 &2.6\% &3.97 &4.24 &6.8\% &4.40 &4.58 &4.0\% \\
Recall@20 &12.72 &13.87 &9.1\% &11.66 &11.92 &2.2\% &11.58 &12.39 &7.0\% &12.73 &13.30 &4.5\% \\
NDCG@20 &7.89 &8.59 &8.9\% &7.24 &7.45 &3.0\% &7.24 &7.77 &7.3\% &7.93 &8.19 &3.4\% \\
\cmidrule(r){1-13}  
\multicolumn{13}{c}{\textsc{Anime}} \\
\cmidrule(r){1-13}  
Recall@10 &21.08 &22.99 &9.1\% &16.44 &17.65 &7.4\% &20.59 &21.80 &5.9\% &20.98 &23.60 &12.5\% \\
NDCG@10 &17.19 &18.85 &9.7\% &13.62 &14.61 &7.3\% &16.83 &17.60 &4.6\% &17.12 &19.31 &12.8\% \\
Recall@20 &33.54 &36.67 &9.3\% &26.45 &28.59 &8.1\% &32.79 &34.97 &6.7\% &33.40 &37.70 &12.9\% \\
NDCG@20 &28.87 &31.58 &9.4\% &22.38 &24.25 &8.4\% &28.03 &29.64 &5.7\% &28.62 &32.42 &13.3\% \\
\cmidrule(r){1-13}  
\multicolumn{13}{c}{\textsc{Gowalla}} \\
\cmidrule(r){1-13}  
Recall@10 &9.56 &9.97 &4.3\% &8.32 &9.04 &8.7\% &9.84 &10.38 &5.5\% &9.31 &9.39 &0.8\% \\
NDCG@10 &5.61 &5.87 &4.7\% &4.87 &5.25 &7.8\% &5.81 &6.12 &5.3\% &5.46 &5.53 &1.3\% \\
Recall@20 &19.29 &20.22 &4.8\% &16.77 &18.23 &8.7\% &20.06 &21.26 &6.0\% &18.61 &18.69 &0.4\% \\
NDCG@20 &10.03 &10.47 &4.4\% &8.67 &9.45 &8.9\% &10.42 &11.03 &5.9\% &9.71 &9.83 &1.2\% \\
\cmidrule(r){1-13}  
\multicolumn{13}{c}{\textsc{Yelp-2018}} \\
\cmidrule(r){1-13}  
Recall@10 &6.81 &7.61 &11.8\% &6.23 &6.74 &8.1\% &7.12 &7.79 &9.5\% &6.60 &7.25 &9.8\% \\
NDCG@10 &3.62 &4.04 &11.7\% &3.33 &3.60 &8.1\% &3.79 &4.14 &9.3\% &3.51 &3.82 &8.9\% \\
Recall@20 &10.35 &11.57 &11.8\% &9.36 &10.21 &9.1\% &10.65 &11.69 &9.7\% &9.96 &10.95 &9.9\% \\
NDCG@20 &6.17 &6.86 &11.2\% &5.67 &6.13 &8.1\% &6.46 &7.08 &9.6\% &5.92 &6.54 &10.6\% \\
\cmidrule(r){1-13}  
\multicolumn{13}{c}{\textsc{MovieLens-1M}} \\
\cmidrule(r){1-13}  
Recall@10 &18.10 &19.82 &9.5\% &15.56 &17.33 &11.4\% &18.01 &19.41 &7.8\% &17.96 &19.60 &9.2\% \\
NDCG@10 &20.15 &22.14 &9.9\% &17.48 &19.37 &10.8\% &20.00 &21.81 &9.1\% &19.89 &21.72 &9.2\% \\
Recall@20 &25.72 &28.15 &9.4\% &22.40 &25.02 &11.7\% &25.89 &27.77 &7.3\% &25.56 &27.81 &8.8\% \\
NDCG@20 &26.84 &29.42 &9.6\% &23.41 &26.13 &11.6\% &26.83 &28.96 &8.0\% &26.69 &29.30 &9.8\% \\
\bottomrule
\end{tabular}
}
\label{tab:rebuttal_table2}
\end{center}
\vspace{-0.1in}
\end{table*}

